E2FL: Equal and Equitable Federated Learning

Federated Learning (FL) enables data owners to train a shared global model without sharing their private data. Unfortunately, FL is susceptible to an intrinsic fairness issue: due to heterogeneity in clients' data distributions, the final trained model can give disproportionate advantages across the participating clients. In this work, we present Equal and Equitable Federated Learning (E2FL) to produce fair federated learning models by preserving two main fairness properties, equity and equality, concurrently. We validate the efficiency and fairness of E2FL in different real-world FL applications, and show that E2FL outperforms existing baselines in terms of the resulting efficiency, fairness of different groups, and fairness among all individual clients.

==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/Design.tex <==
% \clearpage\null
\vspace{-3pt}
\section{\XYZ{}: Design}
% \vspace*{-6pt}
In this section, we provide the design of our Equal and Equitable Federated Learning (\name) algorithm. We first describe how \name
provides equity and then discuss how it provides equality. 
The intuition behind \XYZ{} is to train multiple global models, and first perform a majority vote among the clients' model updates in each group, and then another majority vote among the group models to find the global model.
Algorithm~\ref{alg:FFRL} describes  \XYZ{} training. 


% algorithm that focuses on the equity and then add a variant of it called Equalized FFRL (E-FFRL) to provide both equality and equity.
% In \XYZ{} through awareness, server initialize the random weights and scores (Algorithm~\ref{alg:Awa} line3) using a random seed (\textsc{Seed}) and it also broadcast the seed to all the clients, so they can construct the same weights and scores. 
% In the $t^{th}$ round, \XYZ{} server randomly selects $n$ clients among total $N$ clients, and shares the global rankings $R_{g}^{t}$ with them.
% Client $u$ learns a different local ranking for each group of data it owns, i.e., for group $j$, it learns a specific local ranking $R_{u,j}^t$ starting from the global ranking $R_g^t$ on training data of that group $D_{u}^{tr|A=j}$ (Algorithm~\ref{alg:Awa} line 12). 

% After collecting all local rankings from the selected clients and different groups they own, the server first performs a majority vote on the rankings inside each group to calculate the global ranking for each group $R_{g,j}^{t+1}$ (Algorithm~\ref{alg:Awa} line 18-20). And then it performs a majority vote on the votes of all the groups to calculate the global ranking of next round $R_{g}^{t+1}$ (Algorithm~\ref{alg:Awa} line 21).
% We consider two types of FL based on the clients data belongs to what groups:




% \begin{wrapfigure}{r}{0.6\textwidth} 
% \begin{figure}
%  \centering
%  \footnotesize
%  \vspace{-20pt}
%     \begin{minipage}{0.49\textwidth} 
\begin{algorithm}[h]
\footnotesize
\caption{Equal and Equitable Federated Learning (\name) Algorithm.}\label{alg:FFRL}
\begin{algorithmic}[1]
\footnotesize
\State \textbf{Input:} number of FL rounds $T$, number of local epochs $E$, number of selected users in each round $n$, number of groups $Q$, seed $\textsc{seed}$, learning rate $\eta$, subnetwork size $k$\%
% \State \serverbox{Server: Initialization}
\State $\theta^s, \theta^w \gets$ Initialize random scores and weights of global model $\theta$ using \textsc{seed}
\State $R_{g}^{1} \gets \textsc{ArgSort}(\theta^s)$ \Comment{Sort the initial scores and obtain initial global rankings}
\For{$t \in [1,T]$}
    \State $U \gets$ set of $n$ randomly selected clients out of $N$ total clients
    \For{$u$ in $U$}
        % \State \clientbox{Clients: Local Rankings}
        % \State \mtasks{$R_{u,j\in[q]}^{t} \gets \textsc{AwareLocalRanking}(R_{g}^{t}, D_u^{tr})$} \Comment{Fairness through awareness}
        % \State \onetask{$ R_{u,\hat{j}}^{t} \gets \textsc{UnAwareLocalRanking}(R_{g}^{t}, D_u^{tr})$}  \Comment{Fairness through Unawareness}
        \State $\theta^s, \theta^w \gets $ Initialize scores and weights using \textsc{seed}
        % \State $q=\textsc{identity}(\theta^w, M_{g,q\in[Q]}^{t}, Q, D_u^{tr})$ \Comment{Identity estimation using binary masks of different groups}
        \State If $q$ (group ID) is not known, use Algorithms~\ref{alg:IDEKmeans} and~\ref{alg:IDE} for ID inference (Section~\ref{Sec:main_unkown})
        \State $\theta^s[R_{g}^{t}] \gets \textsc{sort}(\theta^s)$ \Comment{Reorder the scores based on the global ranking}
        \State $\theta_{u}^s \gets$ Edge-PopUp($E, D_u^{tr}, \theta^w, \theta^s, k, \eta$) \Comment{Train local scores on the local training data}
        \State $R_{u, q}^{t} \gets \textsc{ArgSort}(\theta_{u}^s)$ \Comment{Ranking of the client $u$ with estimated group ID: $q$}
        \State \textbf{return} $R_{u,q}^{t}$
    \EndFor
    % \State \serverbox{Server: Majority Vote}
    \State \serverbox{$R_{g, q\in[Q]}^{t+1} \gets \textsc{Vote}(R_{u \in U, q\in[Q]}^{t})$ } \Comment{Majority vote aggregation inside each group}
     \State \serverbox{$R_{g}^{t+1} \gets \textsc{Vote}(R_{g, q\in[Q]}^{t+1})$} \Comment{Majority vote aggregation among all the groups}
\EndFor
\Function{\serverbox{Vote}}{$R_{\{u \in U\}}$ }:
    \State $V \gets \textsc{ArgSort}(R_{\{u \in U\}})$ \Comment{Reputation of each edge in each local ranking}
    \State $A \gets \textsc{Sum}(V)$ \Comment{Sum the reputations}
    \State \textbf{return} $\textsc{ArgSort}(A)$ \Comment{Order of the reputations}
\EndFunction
\end{algorithmic}
\end{algorithm}
%     \end{minipage}
%      \vspace{-17pt}
% \end{figure}
% \end{wrapfigure}





%  \begin{figure*}
%     \centering
%     \includegraphics[width=1.0\textwidth]{Images/unfairness1.jpg}
%     \caption{An example showing difference between FedAvg which provide equality and \XYZ{} which provides Equity. In our system, each vote of Non-Binary user is worth of 3 votes of a Male user and 2 votes of a Female user.}
%     \label{fig:Fairness1}
% \end{figure*}

% Figure~\ref{fig:Fairness1} shows the difference between equality and equity for a scenario that we have three types of voters: a) Male voters, b) Female voters, and c) Non-binary voters. If the voting is considered as averaging (what we have in FedAVG), then the system on the left is trying to provide equality by giving each user a chance to participate in the aggregation of global model. In this case, each user (from all the groups) have one vote which means 1/6 of the global vote. In this scenario, the male voters are in majority, as their vote has three times more effect compared to Non-binary voters. Even the Female voters have a contribution of two times more than Non-binary voters. However, we call this voting system equal as the population with more votes have more power. 

% On the other hand, when we talk about providing equity (right side of~\ref{fig:Fairness1}, we are saying that each group should have an equal contribution to final vote, not each user. We design \XYZ{} to provide equity, by giving all the groups same chance to affect to final vote, and at the same time each voter in each group has same amount of right compared to its peers. In this example, for a fair final vote, first we calculate the vote of each group as $v^{M}, v^{F}, v^{N}$ and vote on these votes to find the final vote $v_g$. Now in final vote, Male voters, Female voters, and Non-binary voters have same effect on the final vote. 




% \paragraphb{FSL as vote: each vote should have equal effect:} For voting in \XYZ{}, we chose FSL voting mechanism for following reasons: We need a voting system that each vote has the same effect as other votes. We cannot consider gradients or model updates as votes, since the direction and magnitude of each parameter has its own effect on the global model. In FSL system, the voters calculate the rankings of edges in a random neural network from most to least important edge. Therefore, each vote is a permutation of integers $i \in [1, d]$ where $d$ is the size of network. 


%  \begin{figure}[H]
%     \centering
%     \includegraphics[width=1.0\textwidth]{Images/unfairness2.jpg}
%     \caption{\XYZ{} design}
%     \label{fig:fflr_design}
% \end{figure}

The key insight used in \name is converting the problem of model weight optimization (in standard FL) to the problem of ranking model edges~ \cite{mozaffari2021frl}. 
In Section~\ref{sec:Rank-based}, we explained how an FL works by training on parameter ranks. 
In \name, each local update (one vote) is a ranking, i.e., a permutation of integers $\in [1, d]$ where $d$ is the size of network layer.
% In \name, we train rankings (compared to weight training in standard FL) which has been suggested in~\cite{mozaffari2021frl}. 
We use rankings because of their intrinsic fairness feature: In rank aggregation, each local ranking has the same impact on the aggregated global ranking. In rank-based FL, all the local rankings are bounded to be a permutation of unique integers $\in [1, d]$. 
For example, for a network layer with $d=3$ parameters, there are only $3!$ possible permutations for local ranking (${[1,2,3], \dots, [3,2,1]}$).
However, in existing standard FL designs, the local updates ($\in \mathbb{R}^d$) have different impacts on the aggregated global model because the direction and magnitude of each parameter update is not bounded to other parameters. 
% We cannot consider gradients or model updates as votes, since the direction and magnitude of each parameter has its own effect on the global model.
% Majority voting in rank aggregation allows more equal contribution from all the participating clients.  

% \paragraphb{In \name aggregation, each vote has equal impact on the final vote.} For voting in \XYZ{}, we chose FRL voting mechanism for following reasons: We need a voting system that each vote has the same effect as other votes.  In FRL system, the voters calculate the rankings of edges in a random neural network from least to most important edges. Therefore, 

In \name, different FL clients gather together to learn a global model, but each one of them belongs to a different group (which could be considered known or unknown). In this section, we assume the clients know their group IDs, and in Section~\ref{Sec:main_unkown}, we explain how the clients can infer their group IDs using the features of rankings when the groups are unknown. In \XYZ{}, the server trains multiple global rankings, each one belonging to a different group. These global group rankings are showing different orders of importance of same supernetwork for different groups from least to most important edges. Each client participates in the training of their group model by sending the local ranking they have. For aggregation, the server performs a majority vote among the local rankings (local votes) in each group, and then performs another majority vote among global group rankings (group votes) to find the global model for the next round (i.e., global ranking that clients will start their training for next \name round).

\paragraphb{Edge-PopUp Algorithm}
The edge-popup (EP) algorithm~\citep{ramanujan2020what} is an optimization method to find supermasks within a large, randomly initialized neural network, i.e., a supernetwork, with performances close to the fully trained supernetwork.
 EP algorithm does not train the weights of the network, instead only decides  the set of edges to keep and removes the rest of the edges (i.e., pop).
Specifically, EP algorithm assigns a positive score  ($\theta^s$) to each of the edges in the supernetwork and updates it.
In \name, each client learns its local scores $\theta_{u}^s$ by using EP on its local data for $E$ local epochs starting from the global scores $\theta^s $.
On forward pass, it selects the top $k\%$ edges with highest scores, where $k$ is the percentage of the total number of edges in the supernetwork that will remain in the final subnetwork. On the backward pass, it updates the scores with the straight-through gradient estimator~\citep{bengio2013estimating}. Algorithm~\ref{alg:edgepop} in Appendix~\ref{sec:EP} presents EP algorithm.
 \begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Images/ICML_FFRL_example_Race.pdf}
    \vspace{-20pt}
    \caption{A single \XYZ{} round with six clients from three groups and a network of 6 edges. Note that all the operations in \name training are performed in a layer-wise manner. 
    }
    % \vspace{5pt}
    \label{fig:fflr_design}
    \vspace{-5pt}
\end{figure}

We detail a round of \XYZ{} training and depict it in Figure~\ref{fig:fflr_design}, where we use a supernetwork with six edges $e_{i\in[0,5]}$ to demonstrate a single \XYZ{} round and consider six clients $C_{j\in[1,6]}$ from three groups (handwriting style A, B, C) who aim to find a subnetwork of size $k$=50\% of the original supernetwork.

%  \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{Images/FFRL_example_Race.drawio_5.pdf}
%     \vspace*{-20pt}
%     \caption{A single \XYZ{} round with six clients from three groups and network of 6 edges. Please note that, all the operations in \name training are performed in a layer-wise manner. 
%     }
%     \vspace{5pt}
%     \label{fig:fflr_design}
%     % \vspace*{-15pt}
% \end{figure*}





\paragraphb{Server: Initialization Phase (Only for round $t=1$)}:
In the first round, the \XYZ{} server chooses a random seed \textsc{Seed} to generate initial random weights $\theta^w$  and scores $\theta^s$ for the global supernetwork $\theta$; note that, $\theta^w$, $\theta^s$, and \textsc{Seed} remain constant during the entire \XYZ{} training. Next, the \XYZ{} server shares  \textsc{Seed} with  \XYZ{} clients, who can then locally reconstruct the initial weights $\theta^w$ and scores $\theta^s$ using \textsc{Seed}. Figure~\ref{fig:fflr_design}-\circled{1} depicts this step. 
Recall that, the goal of \XYZ{} training is to find the most important edges in $\theta^w$ without changing the weights. 
At the beginning, the \XYZ{} server finds the global rankings of the initial random scores , i.e., $R_g^1= \textsc{ArgSort($\theta^s)$}$.
We define \emph{rankings of a vector} as the indices of elements of vector when the vector is sorted from low to high, which is computed using \textsc{ArgSort} function.






\paragraphb{Clients: Calculating the ranks (For each round $t$)}:
In the $t^{th}$ round, \XYZ{} server shares the global rankings $R_{g}^{t}$ with the clients. 
Each of the clients locally reconstructs the weights $\theta^w$'s and scores $\theta^s$'s using \textsc{seed}.
Then, each \XYZ{} client reorders the random scores based on the global rankings, $R_{g}^{t}$. We depict this in Figure~\ref{fig:fflr_design}-\circled{2a}. For instance, the initial global rankings for this round are $R^t_g=[2,3,0,5,1,4]$, meaning that edge $e_4$ should get the highest score ($s_4=1.2$), and edge $e_2$ should get the lowest score ($s_2=0.2$).



Next, each of the clients uses reordered $\theta_u^s$ and finds a subnetwork within $\theta^w$ using edge-popup algorithm~\citep{ramanujan2020what}; to find a subnetwork, they use their local data and $E$ local epochs. Note that, each iteration of edge-popup algorithm updates the scores $\theta_u^s$.
Then client $u$ computes their local rankings $R_{u}^t$ using the final updated scores and \textsc{Argsort}(.), and sends $R_{u,q}^t$ to the server where $q$ is the group identifier. We will explain the group inference methods we propose in Section~\ref{Sec:main_unkown}. 
Figure~\ref{fig:fflr_design}-\circled{2b} shows, for each client, the local rankings they obtained after finding their local subnetwork. For example, rankings of client $C_1$  are $R^t_{1,A}=[4,0,2,3,5,1]$, i.e., $e_4$ is the least important and $e_1$ is the most important edge for $C_1$. Considering desired subnetwork size to be 50\%, $C_1$ uses edges \{3,5,1\} in their final subnetwork in this round.

\paragraphb{Server: Majority Vote  (For each round $t$)}:
The server receives all the local rankings of the clients, i.e., $\{R^t_{1,A}, R^t_{2,A}, R^t_{3,A}, R^t_{4,B}, R^t_{5,B}, R^t_{6,C}\}$. 
Then, it performs a majority vote over all the local rankings inside each group, i.e., $\{A, B, C\}$. We depict this in Figure~\ref{fig:fflr_design}-\circled{3a}.
Note that, for group $q$, the index $i$ in ${R^{t+1}_{g,q}}$  represents the  importance of the edge $i$th for clients in group $q$.
For instance, in Figure~\ref{fig:fflr_design}-\circled{3a}, rankings of $A$ are $R^t_{g,A}=[0,2,4,5,3,1]$ and rankings of $B$ are $R^t_{g,B}=[0,2,3,1,4,5]$, hence the edge $e_1$ is the most important edge for group $A$, while the edge $e_5$ is the most important edge for group $B$. 
Next, the server performs a majority vote over all the group rankings of different groups $\{R^{t+1}_{g,A}, R^{t+1}_{g,B}, R^{t+1}_{g,C}\}$ to find the global ranking $R_{g}^{t+1}$. We depict this in Figure~\ref{fig:fflr_design}-\circled{3b}.


% Note that,  \emph{all  \XYZ{} operations that involve sorting, reordering, and voting are performed in a layer-wise manner}. For instance, the server computes global rankings $R^t_g$ in round $t$ for each layer separately, and consequently, the clients selected in round $t$  reorder their local randomly generated scores $\theta^s$ for each layer separately.  




% \vspace*{-6pt}
% \subsection{\name provides both equality and equity}
% \vspace*{-6pt}

\paragraphb{\name provides both equity and equality.} Equity is not the main goal of existing distributed learning systems because it can hurt the motivation of the majority of clients to  participate in the FL. If we have a learning algorithm that provides equity, it has this constraint to allow the same contribution from all groups (i.e., majorities and minorities). This comes with the price of reducing the performance of the majorities, which can demotivate them to participate to learn a model. 

\name provides both equity and equality. 
In this algorithm, at the final round of the learning, instead of using the global ranking, each group uses its own group global rankings. The global rankings can provide better performances to the majority groups as they have access to more training data, so they can train better group global rankings. 
For example, a client of handwriting style A will use $f(x, \theta^w \bigodot M^{t}_{g,A})$ in their downstream classification task, where $M^{t}_{g,A}$ is the learned binary mask for group A at FL round $t$, and $\theta^w$ is the random weights (initialized randomly and kept fixed), and $x$ is the test input. Note that in \name and its variants, $M^{t}_{g,q}$ is the supermask trained for group $q$ where for top $k$\% of the top rankings of group ranking $R_{g,q}^t$, we put 1's and we set other masks to 0's. 

==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/Equity.tex <==
% \clearpage\null
% \vspace*{-6pt}
\section{Fairness Using Two Lenses: Equity and Equality}
% \vspace*{-6pt}
Fairness in FL can be evaluated from two main perspectives:
a) \emph{Equality} which is fairness between individuals and b) \emph{equity} which is fairness between groups. A group is a set of individuals with the same protected attribute. 
The protected attribute may be known to the clients,  e.g., race, gender, or age. Alternatively, clients may be unaware of their particular group,  e.g., handwriting style (as this needs  clustering clients into groups by someone who has samples from all clients).

% \begin{wrapfigure}{r}{0.6\textwidth}
% \centering
% \vspace*{-12pt}
% % \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.58\textwidth]{Images/Unfariness Race_4.jpg}
%     \vspace*{-10pt}
%     \caption{An example showing two different FL systems with two goals: equality (on left) and equity (on right).}
%     \label{fig:Fairness1}
% % \end{figure}
% \end{wrapfigure}
% \begin{wrapfigure}{r}{0.6\textwidth}
% \centering
% \vspace*{-12pt}
\begin{figure}[htb!]
    \centering
    \includegraphics[width=0.49\textwidth]{Images/Unfariness_Race4.pdf} 
    \vspace{-15pt}
    \caption{An example showing two different FL systems with two goals: equality (on left) and equity (on right).}
    \label{fig:Fairness1}
    \vspace{-10pt}
\end{figure}
% \end{wrapfigure}

Figure~\ref{fig:Fairness1} shows an example of two FL systems where six clients want to learn a global model for prediction of handwritten digits.
These clients have three handwriting styles: \textbf{(A)} normal handwriting style, \textbf{(B)} a little bit rotated handwriting, and \textbf{(C)} 180 degree rotated handwriting (upside-down).
We consider each model update ($\theta^q_u$ for client $u$ in group $q$) has the same effect on updating the global model, so each client update is like a vote. 
In this example, group A has the majority of the voters, and group B and C are in minorities. 
The left part of figure shows an FL in which the goal is providing equality, so we give same chance (one vote) to each client to change the final model by an aggregation such as averaging (e.g., what we have in FedAvg). In this setting, the majority group with higher population (group A) has more influence on the final vote. 
On the other hand, the right part shows an FL in which the goal is providing equity. In this setting, first we aggregate the votes inside each group to find the group votes ($\theta^{A}_g, \theta^{B}_g, \theta^{C}_g$), and then aggregate the group votes to produce the final model. 
In this setting, each client has the same chance (one vote) to influence its own group vote, and finally each group of voters have the same chance (one vote) to influence the final vote.
% Influencing the global model in FL is the same scenario as in our example. 
We define two aspects of fairness in FL as follows: 

% If the voting is considered as averaging (what we have in FedAVG), then the system on the left is trying to provide equality by giving each user a chance to participate in the aggregation of global model. In this case, each user (from all the groups) have one vote which means 1/6 of the global vote. In this scenario, the male voters are in majority, as their vote has three times more effect compared to Non-binary voters. Even the Female voters have a contribution of two times more than Non-binary voters. However, we call this voting system equal as the population with more votes have more power. 

% On the other hand, when we talk about providing equity (right side of~\ref{fig:Fairness1}, we are saying that each group should have an equal contribution to final vote, not each user. We design \XYZ{} to provide equity, by giving all the groups same chance to affect to final vote, and at the same time each voter in each group has same amount of right compared to its peers. In this example, for a fair final vote, first we calculate the vote of each group as $v^{M}, v^{F}, v^{N}$ and vote on these votes to find the final vote $v_g$. Now in final vote, Male voters, Female voters, and Non-binary voters have same effect on the final vote. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.7\textwidth]{Images/unfairness1.jpg}
%     \caption{An example showing difference between FedAvg which provide equality and \XYZ{} which provides Equity. In our system, each vote of Non-Binary user is worth of 3 votes of a Male user and 2 votes of a Female user.}
%     \label{fig:Fairness1}
% \end{figure}





% \subsection{Definitions}
% Current definitions and fairness algorithms in centralized ML cannot be extended into FL because of two reasons: 1) multi-party training ecosystem of FL introduces unique notions of algorithmic bias. 2) the nature of data bias and minority groups is different in FL. We look at the fairness with two lenses:

% \paragraph{Group Fairness notion:}



\paragraphb{Definition 1 (Equality: User-level Fairness):} 
Trained global model $\theta$ is more \emph{equalized} when its performance is more uniform across the individual clients participating in FL, i.e., when  STD$\{F_u(\theta)\}_{u \in [N]}$ is smaller where STD$\{.\}$ is the standard deviation, and $F_u(.)$ denotes the local objective function of client $u$ from $N$ clients. 
Existing fair federated learning literature~\cite{li2019fair, li2020ditto, Smith17, hashimoto2018fairness, zhang2020personalized, mohri2019agnostic, yu2020salvaging} use this definition in their designs.    

\paragraphb{Definition 2 (Equity: Group-level Fairness):}
Trained global model $\theta$ is more \emph{equitable} when its performance is more uniform across the groups, i.e., when 
STD$\{$Avg$\{F_u(\theta)\}_{u \in [q]}\}_{q \in [Q]}$ is smaller where AVG$\{\}_{u \in [q]}$ denotes the average of performances for all the individual clients in the $q$th group, and there are $Q$ total groups. 

% In this notion, we want similar performance for all the groups, instead of all the individual clients where a group is a set of client with similar data distribution.
% An FL algorithm is more fair when distribution of its performance distributions across the clients inside different group is more uniform. It means that each group will get similar treatment.  
% Therefore, an FL model $w$ is more fair, when STD$\{$Avg$\{F_k(w)\}_{k \in [g]}\}_{g \in [G]}$ is less for all the $G$ groups. 


In \name, our goal is providing both equity and equality. To provide equity, an individual client has one vote in their group, and each group has one vote among all the groups. To provide equality, we allow the clients in each group use their group model which represents their training data better.  

 


















==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/Exp.tex <==


% \pagebreak
\vspace{-6pt}
\section{Experiments}
% \vspace*{-6pt}
In this section, we investigate the utility, fairness, and communication cost of \name in two different settings of known and unknown group IDs. 
We use three benchmark datasets widely used in prior works on federated learning application. We run all the experiments for 5 runs with different seeds, and report the average of them. 
Due to space limitations, we defer a detailed discussion of datasets, model architectures, hyperparameters, and the baselines to Appendix~\ref{sec:hyp}. 
% % \begin{wrapfigure}{r}{0.5\textwidth}
% % \centering
% % \vspace{-20pt}
% \begin{figure}[hbt!]
%     \begin{center}
%     \begin{subfigmatrix}{1}
%     \centering
%       \subfigure[Data sample from each group]{
%       \includegraphics[width=0.8\columnwidth]{Images/new_Data.jpg}}
%     \end{subfigmatrix}    
%     \vspace{-6pt}
%     \begin{subfigmatrix}{1}
%     \centering
%       \subfigure[Number of clients in each group]{
%       \includegraphics[width=0.9\columnwidth]{Images/data_FFMML_bar.eps}}
%     \end{subfigmatrix}    
%     \end{center}
%     \vspace*{-15pt}
%     \caption{FairMNISTPerm: a new dataset to investigate equality and equity in FL application.}
%     \label{fig:4Loss1}
%     % \vspace*{-20pt}
% \end{figure}
% % \end{wrapfigure}


\begin{figure}[hbt!]
    \begin{center}
    \begin{subfigmatrix}{1}
    \centering
      \subfigure[Data sample from each group]{
      \includegraphics[width=0.6\columnwidth]{Images/new_Data.jpg}}
    \end{subfigmatrix}    
    \vspace{-6pt}
    \begin{subfigmatrix}{1}
    \centering
      \subfigure[Number of clients in each group]{
      \includegraphics[width=0.9\columnwidth]{Images/data_FFMML_bar.eps}}
    \end{subfigmatrix} 
    % \vspace{-6pt}
    \begin{subfigmatrix}{1}
    \centering
      \subfigure[Final test loss for all the groups]{
      \includegraphics[width=0.9\columnwidth]{Images/LOSS_FFMML_bar_6.eps}}
    \end{subfigmatrix} 
    \end{center}
    \vspace*{-15pt}
    \caption{FairMNISTRotate: a new dataset to investigate equality and equity in FL application.}
    \label{fig:4Loss1}
    % \vspace*{-20pt}
\end{figure}


% \paragraphb{Providing fairness in FL is different from personalization.} \blue{Personalized FL (PFL) algorithms also can reduce the variance of clients' performances by personalizing the global model for each client. However the fair FL algorithms are different from PFL algorithms. The main benefit of PFL is to increase the utility of the global model, and we can use the idea of personalization on top of fairness algorithms too. In PFL algorithms, the clients personalize the received global model by different techniques such as fine-tuning~\cite{yu2020salvaging, mansour2020three, wang2019federated, zhao2018federated}, mixing global and local models~\cite{Smith17,  li2020ditto, hanzely2020federated, deng2020adaptive}, re-weighting~\cite{zhang2020personalized, li2020tilted, mohri2019agnostic}, meta-data learning~\cite{chen2018federated,jiang2019improving,  finn2017model, fallah2020personalized}, and representation learning~\cite{liang2020think, collins2021exploiting}. The idea of these techniques can be added on top of \name to produce higher performance and reduce the variance of the performances. Because of this reason, we compare our work with q-FFL~\cite{li2019fair}, which is a fairness algorithm and can be added to any of the above personalization techniques. }

% \subsection{Experiment Setup}\label{sec:setupp}



% \subsubsection{Datasets and model architectures} \label{app:dataset}


% \paragraphb{MNIST}  is a 10-class class-balanced classification task with 70,000 gray-scale images, each of size 28 × 28. We experiment with LeNet architecture given in Table~\ref{tab:models}. For local training in each \Name{}/FL round, each client uses 2 epochs. 
% For training weights (experiments with FedAvg, SignSGD, TopK), we use SGD optimizer with learning rate of 0.01, momentum of 0.9, weight decay of 1e-4, and batch size 8. For training ranks (experiments with \Name{}), we use SGD with learning rate of 0.4, momentum 0.9, weight decay 1e-4, and batch size 8. 

% \paragraphb{FairMNISTPerm: } 







% \paragraphb{CIFAR10}~\cite{krizhevsky2009learning} is a 10-class classification task with 60,000 RGB images (50,000 for training and 10,000 for testing), each of size 32 × 32. We experiment with a VGG-like architecture given in Table~\ref{tab:models}, which is identical to what \cite{ramanujan2020what} used.
% For local training in each \Name{}/FL round, each client uses 5 epochs.
% For training weights (experiments with FedAvg, SignSGD, TopK), we use SGD with learning rate of 0.1, momentum  of 0.9, weight decay of 1e-4, and batch size of 8. For training ranks (experiments with \Name{}), we optimize SGD with learning rate of 0.4, momentum of 0.9, weight decay of 1e-4, and batch size of 8. 

% For local training in each \Name{}/FL round, each client uses 2 epochs. 
% For training weights (experiments with FedAvg, SignSGD, TopK), we use SGD with learning rate of 0.15, momentum of 0.9, weight decay of 1e-4,  and batch size of 10. For training ranks (experiments with \Name{}), we optimize SGD with learning rate of 0.2, momentum of 0.9, weight decay of 1e-4, and batch size of 10. 

% We optimize the hyperparameters based on \Name{} and other baselines independently.



% \subsubsection{Baseline FL Algorithms}\label{exp_setup:baseline_fl}
% We compare the \XYZ{} with following FL baselines:











% \clearpage\null
% \vspace*{-6pt}
\subsection{Equality vs Equity via \XYZ{}}
% \vspace*{-6pt}
\paragraphb{FairMNISTRotate:} To measure the equity and equality, we release a new dataset for fairness experiments in FL application. 
We note that creating different data distributions by manipulating standard datasets such as MNIST has been widely adopted in the continual research community~\citep{goodfellow2013empirical, kirkpatrick2017overcoming, lopez2017gradient}, therefore, we create this dataset by rotating the images in MNIST for each group. Figure~\ref{fig:4Loss1}a shows image samples in each group, and Figure~\ref{fig:4Loss1}b shows the number of clients in each group.
In this dataset, we assign same number of data samples to 1000 clients with 10 different data distributions (with different number of clients in each group). There are majority groups with large number of clients, e.g., G6 with 257 clients, and there are minority groups with small number of clients, e.g., G1 with 8 clients.  In this dataset G1 and G10 are minorities, and G5 and G6 are in majorities. 


% create 10 groups of clients by assigning normal distribution of MNISTperm
% 1000 users in each group: [8  25  57 147 245 257 164  70  20   7] distributed normally
% the A=0,9 are the under representative, and A=5 is the majority group with 257 users 




% % \begin{wrapfigure}{r}{0.6\textwidth}
% % \centering
% % \vspace{-20pt}
% \begin{figure}[H]
%     \begin{center}
%     \includegraphics[width=0.49\textwidth]{Images/LOSS_FFMML_bar_6.eps}
%     \end{center}
%     \vspace*{-15pt}
%     \caption{Final test loss for all the groups on FairMNISTRotate.}
%     \label{fig:upper}
%     % \vspace*{-10pt}
% \end{figure}
% % \end{wrapfigure}


\begin{table*} [!htb]
\caption{Comparing equality, equity, and communication cost of different variant of FLs on FairMNISTRotate with 1000 clients.} \label{tab:fairMNIST}
\vspace*{-8pt}
\centering
\footnotesize
% \setlength{\extrarowheight}{0.05cm}
% \resizebox{\textwidth}{!}{
\begin{tabular} {|c||c|c|c|c||c|c|c|c||c|c|}
  \hline
  \multirow{3}{*}{Approach }  & \multicolumn{10}{c|}{Metric} \\ \cline{2-11}
  
  & \multicolumn{4}{c|}{Group-level Fairness (Equity) }&\multicolumn{4}{c|}{User-level Fairness (Equality) }  & \multicolumn{2}{c|}{Comm Cost} \\ \cline{2-11}
   & Avg  & \vtop{\hbox{\strut Worst}\hbox{\strut (10\%)}} & \vtop{\hbox{\strut Best}\hbox{\strut (10\%)}} & Variance & Avg & \vtop{\hbox{\strut Worst}\hbox{\strut (10\%)}} & \vtop{\hbox{\strut Best}\hbox{\strut (10\%)}} & Variance & \vtop{\hbox{\strut Up}\hbox{\strut (MB)}} & \vtop{\hbox{\strut Down}\hbox{\strut (MB)}} \\ \cline{1-11}
   
  Local training & 84.78  & 84.28 & 85.35  & 0.11 & 85.03  & 81.36  & 87.78 & 3.44 & 0 & 0 \\ \cline{1-11}
     FedAvg &  93.89 & 81.88 & 98.32  & 31.81 & 97.61  & 92.87 & 98.32  & 4.49 & 6.20 & 6.20\\ \cline{1-11}
  IFCA    &  \textbf{97.78}  & \textbf{95.01} & \textbf{99.08}  &  1.98 & \textbf{98.79}  & \textbf{96.86}  & \textbf{99.08}  & 0.35  & 6.20  &  62.0 \\ \cline{1-11}
  q-FFL &  92.23 & 77.31 & 98.42 & 57.46 & 97.56  & 93.33  & 98.42 &  4.32 & 6.20 & 6.20 \\ \cline{1-11}
%   \textbf{Our \name (GM)} &   95.41 &  91.68 & 97.18 & 3.38 &  96.67 & 94.93 & 97.18 & 0.57 & 4.05  & 5.99 \\ \cline{1-11} 
  \textbf{Our \name} & 96.52  & 93.90  & 97.81 & \textbf{1.63} & 97.48 & 96.07 & 97.81  &  \textbf{0.33} & \textbf{4.05}  & \textbf{5.99} \\ \cline{1-11} 
\hline 
\end{tabular}
% }
\label{tab:MNISTPerm}
% \vspace*{-5pt}
\end{table*}


\begin{table*} [!htb]
\caption{Comparing utility, equality, and communication cost on FEMNIST with 3400 default clients.} \label{tab:FEM}
\vspace*{-8pt}
\centering
% \small
\footnotesize
% \setlength{\extrarowheight}{0.05cm}
% \resizebox{\textwidth}{!}{
\begin{tabular} {|c||c|c|c|c||c|c||}
  \hline
  \multirow{3}{*}{Approach }  & \multicolumn{6}{c|}{Metric} \\ \cline{2-7}
  
  & \multicolumn{4}{c|}{User-level Fairness (Equality) } & \multicolumn{2}{c|}{Communication Cost} \\ \cline{2-7}
   & Average  & \vtop{\hbox{\strut Worst}\hbox{\strut (10\%)}} & \vtop{\hbox{\strut Best}\hbox{\strut (10\%)}} & Variance & \vtop{\hbox{\strut Up}\hbox{\strut (MB)}} & \vtop{\hbox{\strut Down}\hbox{\strut (MB)}} \\ \cline{1-7}
   
  Local training &  68.74 & 44.45  & 87.41 & 154.50 & 0 & 0 \\ \cline{1-7}
     FedAvg & 85.50 & 63.51  & 99.39  & 108.24 & 6.23 & 6.23\\ \cline{1-7}
  q-FFL & 84.40  &64.09  & 99.14  & 100.80 & 6.23 & 6.23 \\ \cline{1-7}
%   Our \name (GM) - using OneShot & 83.53  & 60.29  & 98.38 & 122.32 & 4.06  & 6.01 \\ \cline{1-7}
%   Our \name (GM) - using Rank Clustering & 84.69 & 62.75 & 98.91 &  108.57 &  4.06  & 4.06 \\ \cline{1-7}
%     Our \name (GM) - using Lowest Loss &  84.49 & 62.65 & 98.71 & 108.78   & 4.06  & 6.01 \\ \cline{1-7}
    \textbf{Our \name (OneShot)} & 83.52   & 60.37  & 98.31 & 121.44 & 4.06  & 6.01 \\ \cline{1-7} 
    \textbf{Our \name (Rank Clustering)} &  87.40 & 67.30 & \textbf{100} &   88.54 &  \textbf{4.06 } & \textbf{4.06} \\ \cline{1-7}
  \textbf{Our \name (Lowest Loss)} & \textbf{87.93}  & \textbf{68.59}  & 99.96  & \textbf{81.88}  & 4.06  & 6.01 \\ \cline{1-7}
   
  
\hline \hline
\end{tabular}
% }

% \vspace*{-8pt}
\end{table*}

% We compare FFRL and E-FFRL with 

In Figure~\ref{fig:4Loss1}c, we compare the performance of different FL algorithms by plotting the test loss of the global trained model for all the ten groups. 
In addition to the results of \name, which is the performance of the global ranking trained for each group, we report the results of the global model as \name (GM).
%We also provide the performance of the global model throughout the FL learning for G1 (a minority group) and G6 (a majority group) in Appendix~\ref{sec:exp2}.
We additionally compare the utility, equity, equality, and communication cost of these baselines in Table~\ref{tab:fairMNIST}.  

Our experimental results on FairMNISTRotate show that: 
\textbf{(1)}\textbf{ clients have motivation to participate in FL}. All the groups including minorities and majorities get benefit by participating in an FL framework. If each client wants to learn a local model on its local data, they cannot use other clients' knowledge, so their local models perform poorly. 
\textbf{(2)} \textbf{FedAvg gives more attention to majority groups.} FedAvg focuses on the clients from majority groups. Client from majority groups can get more benefit by participating in FedAvg as they have more chance to be selected in each round, so they have more impact on the global model. 
FedAvg can achieve 97.61\% mean test accuracy for all the individual clients (i.e., user-level fairness), but the mean of accuracies for groups is low as 93.89\% which shows that this learning paradigm is focusing on user-level fairness more than on group-based fairness (equity).
\textbf{(3)} \textbf{q-FFL improves equality while worsens equity}. q-FFL is helping the majority groups by ignoring the minorities. q-FFL is a user-level fairness framework, so it makes the results more fair compared to FedAvg in equality; however it produces more unfair results compared in equity. 
\textbf{(4)} \textbf{Training 10 different FLs (i.e., IFCA) is not the best situation for the minorities}. It is important that all the groups in FL share their knowledge.  Figure~\ref{fig:4Loss1}c shows that groups G1, G2, and G10 cannot get similar benefits by participating in IFCA since there is no shared knowledge, and these clients have access to limited data. There is another drawback for IFCA compared to \name which is communication cost. \name clients need to get the binary masks compared to IFCA that they need to get actual weight parameters so \name consumes 5.99 MB compared to IFCA which needs 62.0 MB for download bandwidth. Additionally, IFCA cannot get benefit by our entropy approaches since they are designed for binary masks. 
% b) group-ID estimation converge, as we show in Section, sometimes lowest loss cannot be a good indicator. at the end, E-FFRL can achieve even more fair results compared to IFCA.  
\textbf{(5)} \textbf{\name is providing equality and equity}. While q-FFL reduces the variance of accuracies for all the clients by 4\% while it increases the variance between groups by 81\% compared to FedAvg. On the other hand our algorithm can reduce both variance of clients and groups by 93\% and 95\% respectively compared to FedAvg




% \paragraphb{ Local vs. FedAvg: incentive to participate in FL.}  Figure~\ref{fig:Allloss}(a) shows that all the groups including minorities and majorities get benefit by participating in an FL framework. Table~\ref{tab:MNISTPerm} also shows that if each client wants to learn a local model on its local data, they cannot use other clients' knowledge, so their local models perform poorly. This comparison shows that the clients have this incentive to participate in FL to get a more accurate model. For example, the local models can produce an average test accuracies for all the individual clients as 85.03\% which is much lower than 97.61\% which can be achieved by participating in FedAVG. 


% \paragraphb{FedAVG gives more attention to majority groups:} We note from Figure~\ref{fig:Allloss}(a) that FedAvg focuses on the clients from majority groups. Client from majority groups can get more benefit by participating in FedAvg as they have more chance to be selected in each round, they have more influence on the global model. 
% Table~\ref{tab:MNISTPerm} also shows that FedAvg can achieve 97.61\% mean test accuracy for all the individual clients (i.e., user-level fairness), but the mean of accuracies for groups is low as 93.89\% which shows that this learning paradigm is focusing on user-level fairness more than on group-based fairness (equity).

% \paragraphb{QFFL improves equality while worsen equity: QFFL is helping the majority groups by ignoring the minorities.} QFFL is a user-level fairness framework, so we can see from Table~\ref{tab:MNISTPerm} that it makes the results more fair compared to Fedavg in equality; however it produces more unfair results compared to equity. 

% \paragraphb{Training 10 different FLs (i.e., IFCA) is not the best situation for the minorities: It is important that all the groups share their knowledge.}  Figure~\ref{fig:Allloss}(a) shows that groups G1, G2, and G10 cannot get similar benefit by participating in IFCA since there is no shared knowledge, and these clients have access to limited data.  IFCA can produce very good results but there are two main drawback for this framework: a) communication cost: FFRL and E-FFRL needs to get the binary masks compared to IFCA that needs to get the weight parameters so we have 5.99 MB comapred to 62.0 MB. b) group-ID estimation converge, as we show in Section, sometimes lowest loss cannot be a good indicator. at the end, E-FFRL can achieve even more fair results compared to IFCA.  

% \paragraphb{E-FFRL is providing equality and equity.} E-FFRL is a combination of equlity and equity, so ..






% \name when group IDs are Unknown


\vspace{-3pt}
\subsection{\name when Group IDs are Unknown}
% \vspace{-6pt}
In this section, we provide experimental results on the FEMNIST~\citep{DBLP:journals/corr/abs-1812-01097} which is a character recognition classification task distributed over 3,400 clients. 
At first, it seems that data distribution among all the clients are similar as all of them are classifying handwritten letters or digits, but there might be hidden groups of clients among these 3400 clients with even more similar handwriting styles.  In this section, we report the performance of \name with different group inference approaches.
% want to find different groups of clients among these clients, and apply FFRL and E-FFRL on top of them. 
% , 62 classes (52 for upper and lower case letters and 10 for digits), and 671,585 gray-scale images. Each client has data of their own handwritten digits or letters. We use LeNet architecture given in Table~\ref{tab:models}. 




In Table~\ref{tab:FEM}, we compare the performance and fairness of different FL algorithms on FEMNIST. We show the user-level fairness (equality) metrics, as there are not specific groups defined for this dataset.
Our experimental results show that:
\textbf{(1)} Training on local data compared to FedAvg does not provide utility, thus all the clients have incentive to  participate in the FL to get more accurate models. \textbf{(2)} q-FFL~\cite{li2019fair} can provide more equal results by reducing the variance by 7\% with cost of reducing the accuracy by 1.10\%. The reason behind this accuracy reduction is that q-FFL gives more attention to making the clients performances more uniform for the clients in majority groups, so it is using smaller portion of the knowledge from minorities . 
\textbf{(3)} \name shows clear advantage over other algorithms, it can provide both utility and fairness. As the groups are unknown in FEMNIST, we use three different approaches of group inference. For Lowest Loss and OneShot approaches, we use 2 static groups, and for rank clustering we use 5 clusters. We also report more details of 2, 3, 4, and 5 clusters in Appendix~\ref{sec:rankclusterExp} Table~\ref{tab:Kmeans2}. 
\name has good features from both worlds: it can improves the utility and fairness together: EFFL increases the average of accuracies by 2.5\% and reduces the variance of clients by 24\%. These benefits are coming from a) \emph{training multiple models each for one group}, and b) \emph{using knowledge of all the participating clients for all the clients by combining all the group models into one global model}. \textbf{(4)} Lowest Loss and rank clustering perform better than OneShot inference approach because in OneShot we have just one forward and backward passes compared to other methods that needs more operations. 
% \paragraphb{Local vs FedAvg}

% \paragraphb{QFFL vs Fedvg}

% \paragraphb{FFRL with different methods of inference}

% \paragraphb{E-FFRL vs FFRL}


% \begin{figure*}[ht]
% \centering
% \begin{subfigmatrix}{2}
% \centering
%   \subfigure[FedAvg]{
%   \includegraphics[width=1\columnwidth]{Images/fedavg_epochs_loss.eps}}
%   \subfigure[XYZ]{
%   \includegraphics[width=1\columnwidth]{Images/XYZ_epochs_loss.eps}}
% \end{subfigmatrix}    
% \begin{subfigmatrix}{2}
% \centering
%   \subfigure[GXYZ]{
%   \includegraphics[width=1\columnwidth]{Images/GXYZ_epochs_loss.eps}}
%   \subfigure[IFCA]{
%   \includegraphics[width=1\columnwidth]{Images/IFCA_epochs_loss.eps}}
% \end{subfigmatrix}    
% \caption{Fairness}
% \label{fig:4Loss}
% \end{figure*}




% \subsubsection{Results}

%  \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=1.0\textwidth]{Images/LOSS_FFMML_bar.eps}
%     \caption{\textbf{fairness on test acc}}
%     \label{fig:Loss_all}
% \end{figure*}






% \begin{table*} [ht]
% \caption{Comparing performance and communication cost of different variant of FSL with different compression methods when cross-device FL is used. \textbf{MNISTPerm with fairness through unawareness}} \label{tab:comm}
% \centering
% \footnotesize
% \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {|c||c|c|c|c||c|c|c|c||c|c||}
%   \hline
%   \multirow{3}{*}{Approach }  & \multicolumn{10}{c|}{Metric} \\ \cline{2-11}
  
%   & \multicolumn{4}{c|}{Group-level Fairness (Equity) }&\multicolumn{4}{c|}{User-level Fairness (Equlity) }  & \multicolumn{2}{c|}{Communication Cost} \\ \cline{2-11}
%   & \vtop{\hbox{\strut Average}\hbox{\strut (\%)}}  & \vtop{\hbox{\strut Worst 10\%}\hbox{\strut (\%)}} & \vtop{\hbox{\strut Best 10\% }\hbox{\strut (\%)}} & Variance & \vtop{\hbox{\strut Average}\hbox{\strut (\%)}} & \vtop{\hbox{\strut Worst 10\%}\hbox{\strut (\%)}} & \vtop{\hbox{\strut Best 10\%}\hbox{\strut (\%)}} & Variance & \vtop{\hbox{\strut Up}\hbox{\strut (MB)}} & \vtop{\hbox{\strut Down}\hbox{\strut (MB)}} \\ \cline{1-11}
   
%   Local & 84.78 $\pm$ 0.18 & 84.28 $\pm$ 0.02 & 85.35 $\pm$ 0.02 & 0.1117 $\pm$ 0.01  & 85.03 $\pm$ 0.01 & 81.36 $\pm$ 0.01 & 87.78 $\pm$ 0.02 & 3.44 $\pm$ 0.01 & 0 & 0 \\ \cline{1-11}
%      FedAvg &  94.71 $\pm$ 0.09 & 85.45 $\pm$ 0.53 & 98.58 $\pm$ 0.06 & 19.96 $\pm$ 1.26 & 97.79 $\pm$ 0.02 & 93.70 $\pm$ 0.08 & 98.58 $\pm$ 0.06 & 3.15 $\pm$ 0.14 & 6.20 & 6.20\\ \cline{1-11}
%   \vtop{\hbox{\strut IFCA}\hbox{\strut HypCluster}}     &  97.78 $\pm$ 0.02 & 95.01 $\pm$ 0.16 & 99.08 $\pm$ 0.05 &  1.98 $\pm$ 0.10 & 98.79 $\pm$ 0.01 & 96.86 $\pm$ 1.06 & 99.08 $\pm$ 0.05 & 0.35 $\pm$ 0.01 & 6.20  &  62.0 \\ \cline{1-11}
%   q-FFL &  89.80 $\pm$ 0.16 & 68.29 $\pm$ 0.48 & 98.58 $\pm$ 0.01 & 112.34 $\pm$ 5.67 & 97.38 $\pm$ 0.01 & 90.99 $\pm$ 0.14 & 98.58 $\pm$ 0.01 & 9.24 $\pm$ 0.30 & & \\ \cline{1-11}
%   \XYZ{} &    &   & & & & & & & 4.05  & 5.99 \\ \cline{1-11} 
%   G\XYZ{} &   &   & & & & & &  & 4.05  & 5.99 \\ \cline{1-11} 
% \hline \hline
% \end{tabular}
% \end{table*}






% \begin{table*} [ht]
% \caption{FEMNIST} \label{tab:comm}
% \centering
% % \small
% \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {|c||c|c|c|c||c|c||}
%   \hline
%   \multirow{3}{*}{Approach }  & \multicolumn{6}{c|}{Metric} \\ \cline{2-7}
  
%   & \multicolumn{4}{c|}{User-level Fairness (Equality) } & \multicolumn{2}{c|}{Communication Cost} \\ \cline{2-7}
%   & \vtop{\hbox{\strut Average}\hbox{\strut (\%)}}  & \vtop{\hbox{\strut Worst 10\%}\hbox{\strut (\%)}} & \vtop{\hbox{\strut Best 10\% }\hbox{\strut (\%)}} & Variance & \vtop{\hbox{\strut Up}\hbox{\strut (MB)}} & \vtop{\hbox{\strut Down}\hbox{\strut (MB)}} \\ \cline{1-7}
   
%   Local &  68.74 $\pm$ 0.04 & 44.45 $\pm$ 0.16 & 87.41 $\pm$ 0.12 & 154.50 $\pm$ 1.43 & 0 & 0 \\ \cline{1-7}
%      FedAvg & 85.50 $\pm$ 0.14 & 63.51 $\pm$ 0.32 & 99.39 $\pm$ 0.07 & 108.24 $\pm$ 1.55 & 6.20 & 6.20\\ \cline{1-7}
%   q-FFL & 84.40 $\pm$ 0.02  &64.09 $\pm$ 0.08 & 99.14 $\pm$ 0.05  & 100.80 $\pm$ 0.25 &  & \\ \cline{1-7}
%   \XYZ{} (clusering)&    &   & & &  4.05  & 5.99 \\ \cline{1-7} 
%   G\XYZ{} (clustering)  &   &   & &   & 4.05  & 5.99 \\ \cline{1-7}
%     \XYZ{} (lowest loss) &  84.49 $\pm$ 0.11 & 62.65 $\pm$ 0.87 & 98.71 $\pm$ 0.12 & 108.78 $\pm$ 5.93  & 4.05  & 5.99 \\ \cline{1-7} 
%   G\XYZ{}  (lowest loss) & 87.93 $\pm$ 0.07  & 68.59 $\pm$ 0.43  & 99.96 $\pm$ 0.05 & 81.88 $\pm$ 2.49 & 4.05  & 5.99 \\ \cline{1-7}
%     \XYZ{} (oneshot) &    &   & &  & 4.05  & 5.99 \\ \cline{1-7} 
%   G\XYZ{} (oneshot) &   &   & & & 4.05  & 5.99 \\ \cline{1-7}
% \hline \hline
% \end{tabular}
% \end{table*}



% \begin{table} [ht]
% \caption{Comparing performance and communication cost of different variant of FSL with different compression methods when cross-device FL is used. \textbf{MNISTPerm with fairness through unawareness}} \label{tab:comm}
% \centering
% \small
% \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {|c||c|c|c|c|c||}
%   \hline
%   \multirow{3}{*}{Approach }  & \multicolumn{5}{c|}{Metric} \\ \cline{2-6}
  
%   & \multicolumn{2}{c|}{Group-level Accs}& User-level Accs & \multicolumn{2}{c|}{Communication Cost} \\ \cline{2-6}
  
%   & Mean (\%) & STD (\%) & STD (\%) & Up (MB) & Down (MB) \\ \cline{1-6}
%   Local & 85.18 & 0.19 & & 0 & 0 \\ \cline{1-6}
%      FedAvg & 94.0 & 5.33 & & 6.20 & 6.20\\ \cline{1-6}
%   \vtop{\hbox{\strut IFCA}\hbox{\strut HypCluster}}     & 97.74 & 1.48 & & 6.20  &  62.0 \\ \cline{1-6}
%   q-FFL &  & & &  & \\ \cline{1-6}
% %   MOCHA  &   &  &  &  &   & \\ \cline{1-7}   
% %   q-ffl  &   &  &  &  &   & \\ \cline{1-7}   
%   \XYZ{} &   94.41 &  1.28 & & 4.05  & 5.99 \\ \cline{1-6} 
%   G\XYZ{} & 96.48  & 1.04  & & 4.05  & 5.99 \\ \cline{1-6} 
% \hline \hline
% \end{tabular}
% \end{table}



















 
% We use dirichlet to distribute the data samples. 

% \begin{equation}
% EOD=Pr(\hat{Y}=1|A=0, Y=1)-Pr(\hat{Y}=1|A=1, Y=1)
% \end{equation}


% \begin{equation}
% DI=F1(W_g | A=0)- F1(W_g | A=1)
% \end{equation}

% \subsubsection{Baselines}

% Both server and clients use the Singed Kaiming Constant algorithm~\citep{ramanujan2020what} to generate random weights and the Kaiming Uniform algorithm~\citep{he2015delving} to generate random scores.


% We use the same seed to initialize weights and scores.


% \subsubsection{Results}





% \red{two tables one for normal test and one for fair test}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Images/gednderE.eps}
%     \caption{\textbf{fairness on test acc}}
%     \label{table:EOD}
% \end{figure}
  
  
% Table~\ref{table:EOD}: \\
% 1- fedfair works when data is non-iid; in case of iid (cross-silo), it is worse than the fedavg; for non-iid it decreases the accuracy
 
% Figure~\ref{fig:EODvsE}: E=25\\
% 1- first work that with increasing acc EOD does not change or worsen \\











\paragraphb{Miscellaneous Discussions}
Due to space limitations, we defer detailed discussion of ablation studies of \name to Appendix.
In Appendix~\ref{sec:adultexp}, we consider adult census income dataset which is commonly used in fair machine learning literature. In this experiment, we give data samples of different groups to different clients. In Appendix~\ref{sec:rankexpMNIST}, we evaluate the performance of different group inference approaches we introduced on FairMNISTRotate and FEMNIST. 



% \vspace{-6pt}
% \subsection{Miscellaneous Discussions}
% \vspace{-6pt}
% Due to space limitations, we defer a detailed discussion of ablation studies of \name to Appendix and below give their important takeaways. 
% In Appendix~\ref{sec:adultexp}, we consider adult census income dataset~\citep{kohavi1996scaling} which is commonly used in fair machine learning literature. 


% \paragraphb{Fairness with multiple groups in each client:}
% We also provide additional experimental results on adult census income dataset~\citep{kohavi1996scaling} which is commonly used in fair machine learning literature. 
% We consider gender as the protected attribute where we consider male samples as the privileged group and female samples as unprivileged samples.
% This dataset is biased towards male group where the male group has a higher chance of 31.4\% of getting positive while female group has a chance of 11.3\%. We defer our experimental results to Appendix~\ref{sec:adultexp}. 
% In Table~\ref{tab:adult1}, we show that \name can improve the fairness with low cost on the accuracy of the global model in this setting.


% \paragraphb{Rank clustering approach performance:} 
% Table~\ref{tab:KmeansMNIST} in Appendix~\ref{sec:rankexpMNIST} shows the accuracy of the Ranking clustering approach when 1000 clients with FairMNISTPerm data train their local ranking for 2 local epochs. From this table we can see that with larger rankings, we can predict group-ID with higher accuracy. We also provide results of equity and equality of \name on FEMNIST for different number of clusters in Table~\ref{tab:Kmeans}.

% \paragraphb{Performance of group inference approaches on client-side:}
% Figure~\ref{fig:Acc1} in Appendix~\ref{sec:client_based_exp} shows the accuracy of group inference by three methods we proposed for client side for the 300 initial global epochs of \name trained on FairMNISTPerm. We can see that lowest loss method can produce more accurate results compared to Binary and one-shot method with cost of calculating $k$ forward passes. Also Binary method can produce better results compared to one-shot as it requires only one forward and backward passes to determine the group ID. 

% \paragraphb{Rank clustering with different number of groups} Appendix~\ref{sec:rankclusterExp} Table~\ref{tab:Kmeans}


% In Appendix~\ref{}, we analyze different approaches we propose for identity inference. 





% \clearpage\null
% \subsection{\XYZ{} Fairness through unawareness: group ID estimation}
% In this section we analyze different approaches we propose for identity inference. 
% Table~\ref{tab:KmeansMNIST} shows the accuracy of the Ranking clustering method when 1000 clients with FairMNISTPerm data train their local ranking for 2 local epochs. From this table we can see that with larger number of rankings, we can predict better group-ID. 
% % When there is no explicit definition for sensitive attribute:

% % \paragraphb{Server Side: Clustering}

% \begin{wrapfigure}{r}{0.4\textwidth} 
%  \centering
%  \footnotesize
%  \vspace{-40pt}
%     \begin{minipage}{0.3\textwidth} 
% \begin{table}[H]
% % \begin{table} [H]
% \caption{KMeans clustering E=2 for 10 tries} \label{tab:KmeansMNIST}
% \centering
% \footnotesize
% % \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {c|c||c}
%   \hline
%   Layer & No Params  & Accuracy \\ \cline{1-3}
%      Conv1 & 288 &  91.78  \\ \cline{1-3}
%      Conv2 & 18432 &  94.94  \\ \cline{1-3}
%      FC1 & 1605632 &  93.76  \\ \cline{1-3}
%      FC2 & 1280 &  91.99  \\ \cline{1-3}
%      ALL & 1625632 &  93.21 \\ \cline{1-3}
% \hline \hline
% \end{tabular}
% \end{table}
% \vspace{-10pt}
%     \end{minipage}
% \end{wrapfigure}




% \begin{table} [ht]
% \caption{KMeans clustering E=2 for 10 tries} \label{tab:Kmeans}
% \centering
% \footnotesize
% % \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {c|c||c}
%   \hline
%   Layer & No Params  & Accuracy \\ \cline{1-3}
%      Conv1 & 288 &  91.78 $\pm$ 2.98 \\ \cline{1-3}
%      Conv2 & 18432 &  94.94 $\pm$ 2.41 \\ \cline{1-3}
%      FC1 & 1605632 &  93.76 $\pm$ 3.92  \\ \cline{1-3}
%      FC2 & 1280 &  91.99 $\pm$ 3.18  \\ \cline{1-3}
%      ALL & 1625632 &  93.21 $\pm$ 3.20 \\ \cline{1-3}
% \hline \hline
% \end{tabular}
% \end{table}




% \paragraphb{Client Side: lowest loss}

% \paragraphb{Client Side: Binary Search}

% \paragraphb{Client Side: One Shot Estimation}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Images/Est1.eps}
%     \caption{\textbf{for 100 initial epochs, three lines for each approach, x-axis: global epoch, y-axis, accuracy of selected ID}}
%     \label{table:EOD}
% \end{figure}

% Figure~\ref{fig:Acc1} shows the accuracy of group inference by three methods we proposed for client side for the 300 initial global epochs of FFRL. We can see that lowest loss method can produce more accurate results compared to Binary and one-shot method with cost of calculating $k$ forward passes. Also Binary method can produce better results compared to one-shot as it requires only one forward and backward passes to determine the group ID. 



% Due to space limitations, we defer a detailed discussion of ablation studies of group inference to Appendix~\ref{app}.

% \begin{table} [ht]
% \caption{Comparing time complexities of ID estimation approaches} \label{tab:comm}
% \centering
% \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {|c||c||}
%   \hline
%   \multirow{1}{*}{Approach }  & Time Complexity \\ \hline
%   Lowest Loss Method & O(k) forward passes \\ \hline
%   Binary Search & O($\log k$) forward and backward passes \\ \hline
%   OneShot inference & O(1) forward and backward passes \\ \hline
% \end{tabular}
% \end{table}




% \subsection{\XYZ{} Fairness through unawareness: Real data with unknown group ID}
% \begin{table} [ht]
% \caption{FEMNIST (3400 clients) with two groups lr=0.05(0.999)E2} \label{tab:comm}
% \centering
% \small
% \setlength{\extrarowheight}{0.05cm}
% \begin{tabular} {|c||c|c|c|c|c||}
%   \hline
%   \multirow{3}{*}{Approach }  & \multicolumn{5}{c|}{Metric} \\ \cline{2-6}
  
%   & \multicolumn{2}{c|}{\vtop{\hbox{\strut User-level}\hbox{\strut Accuracy}}}& \multicolumn{1}{c|}{\vtop{\hbox{\strut Group-level}\hbox{\strut Accuracy}}}& \multicolumn{2}{c|}{Communication Cost} \\ \cline{2-6}
  
%   & Mean (\%) & STD (\%) & STD (\%) & Up (MB) & Down (MB) \\ \cline{1-6}
%      FedAvg & 85.8 &  10.2 &  -  & 6.23 & 6.23\\ \cline{1-6}
% %   MOCHA  &   &  &  &  &   & \\ \cline{1-7}   
% %   q-ffl  &   &  &  &  &   & \\ \cline{1-7}   
%   \XYZ{} &  83.62 & 10.37  &   1.73 &  4.06  & 4.45\\ \cline{1-6} 
%   G\XYZ{} & 87.91& 9.18  & 0.71 &  4.06 & 4.45 \\ \cline{1-6} 
% \hline \hline
% \end{tabular}
% \end{table}


























% \clearpage\null
% \subsection{Fairness through awareness (cross-silo)}




==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/RelBG.tex <==
% \vspace*{-6pt}
\section{Background}
% \vspace*{-6pt}

% \vspace*{-6pt}
\paragraph{Federated Learning:}
% \vspace*{-6pt}
In FL~\citep{mcmahan2017communication, kairouz2019advances, konevcny2016federated}, 
$N$ clients collaborate to train a global model  without directly sharing their data. 
In  round $t$, the service provider (server) selects $n$ out of $N$ total clients and  sends them the most recent global model $\theta^t$. Each client trains a local model for $E$ local epochs on their data starting from the $\theta^t$ using stochastic gradient descent (SGD). Then the client  sends back the calculated gradients to the server. The server then aggregates the collected gradients and  updates the global model for the next round.
% 
% FL can be either cross-device or cross-silo~\citep{kairouz2019advances}. In cross-device FL, N is large (from few thousands to billions) and only a
% small fraction of clients is chosen in each FL training round, i.e., $n \ll N$. By contrast, in cross-silo FL, N is moderate (up to 100) and all clients are chosen in each round, i.e., $n = N$. 

% In this work, we evaluate the performance of FSL and other FL baselines for cross-device FL under realistic production FL settings.





% \vspace*{-6pt}
\paragraph{Rank-based Federated  Learning:}\label{sec:Rank-based}
% \vspace*{-6pt}
Federated Rank Learning (FRL)~\cite{mozaffari2021frl} is an approach to perform FL that is built on a novel learning paradigm called \emph{supermasks}~\citep{DBLP:conf/nips/ZhouLLY19, ramanujan2020what}.
Specifically, in FRL, clients collaborate  to find a \emph{subnetwork} within a \emph{randomly initialized} neural network (the supernetwork), where this is in contrast to conventional FL where clients collaborate to \emph{train} neural network parameter weights.
The goal of training in FRL is to collaboratively identify a supermask $M_g$, which is a binary mask of 1's and 0's, that is superimposed on the random neural network to obtain the final subnetwork, i.e., $\theta^w \bigodot M_g$ where $\theta^w$ is showing the weight parameters for supernetwork.
$M_g$ contains the edges of top $k$ ranks, i.e., edges in top $k$ ranks (layer-wise) get '1' in the binary mask, and others get '0' in the mask. We use $k=50\%$ in this work to find a subnetwork of 50\% of the original size.
The subnetwork is then used for downstream tasks, e.g., image classification, hence it is equivalent to the global model in conventional FL. Note that in entire FRL training, weights of the network ($\theta^w$) do not change. 


More specifically, 
each  FRL client computes the importance of the edges of the supernetwork based on their local data. The importance of the edges is represented as a ranking vector. 
Each FRL client will use the edge-popup algorithm~\citep{ramanujan2020what} and their data to compute their local rankings (the edge-popup algorithm aims at learning which edges in the random network are more important over the other edges by minimizing the loss of the subnetwork on their local data). 
%Algorithm~\ref{alg:edgepop} in Appendix~\ref{sec:EP} shows how edge-popup works by updating a set of scores $\theta^s$ (the importance of the edges in the supernetwork).
Each client then will send their local edge ranking to the server.
Finally, the FRL server uses a \emph{voting mechanism} to aggregate client rankings into a  supermask, which represents which edges of the random neural network (the supernetwork) will form the global subnetwork. 
Specifically, the FRL server uses Borda count rank aggregation method~\cite{emerson2013original} where it gives a reputation to each edge for each ranking, sums the reputations, and sorts them from least to most to find the global ranking.
We defer further details of FRL and edge-popup Algorithms to Appendix~\ref{sec:FRL}. 


% \subsection{Fair Federated Learning}


==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/UnAwareness.tex <==
% \vspace*{-6pt}
\section{\name when Group IDs are Unknown}\label{Sec:main_unkown}
% \vspace*{-6pt}
In the previous section, we assumed that the clients know their group IDs.
In this section, we explain the approaches the server or a client can utilize to estimate the group IDs when the groups are unknown.
In this setting, there are federated clients that have small amount of data with no known protected attribute. For instance, people with their own style of handwriting want to learn a global model by learning a local model on the images of their handwriting. The clients have no knowledge about their style as it is not something to be identified. It is not even possible to announce that clients with similar style collaborate with each other. This type of scenario usually happens in cross-device setting, where each user has a small dataset and there are so many clients in the system. 
For the server-side approach, the server clusters the local rankings into different groups and assigns a group ID to each client. For client-side approaches, each client should estimate its own group ID using the binary masks learned so far (Algorithm~\ref{alg:FFRL} line 8).
% In our experiments we consider two different settings as follows: 

% \paragraphb{Setting I: unknown protected attribute:} 


% \paragraphb{Setting II: known protected attribute: }
% In this setting, all data samples located at each federated user have a feature called \emph{protected attribute}. For example, data are collected from male and female users, so the protected attribute is gender.




% for example, they know what handwriting style they have. In this section, we discuss how FFRL works when the clients do not know their group ID. 


% In this section and our experiments, we assume we have a fixed number of groups $Q$, however, in Appendix~\ref{sec:qupdate}, we will explain when and how to ask the server to create a new group if the client feels that they do not belong to any of the existing groups.

\paragraphb{Communication Cost of \XYZ{} when group IDs are unknown:} Please note that for finding the best group ID at the client-side, there is no need to send all the group rankings (e.g., $\{R^{t+1}_{g,A}, R^{t+1}_{g,B}, R^{t+1}_{g,C}\}$ in our example) to the clients. As we mentioned before, in \name each ranking (local or global) can be converted to a binary mask of '0's and '1's that is superimposed on the random weights (i.e., supermask). Thus, the server only broadcasts the binary masks of groups (e.g., $\{M^{t+1}_{g,A}, M^{t+1}_{g,B}, M^{t+1}_{g,C}\}$ in our example) to the clients so they can estimate their group ID where they belong to.




















































% \subsection{Group ID Estimation} \label{sec:IDestimation}


% Algorithm~\ref{alg:IDE} describes these methods. We also provide explanation what a client should if none of the existing groups does not match with its training data. 


% \vspace*{-6pt}
\subsection{Server-side:  Rank Clustering}
% \vspace*{-6pt}
Working with rankings enables us to design an efficient algorithm to cluster the local rankings. 
Clustering rankings is more efficient than clustering the model weight updates in standard FL. The main reason is that rankings are from a \emph{discrete} space ($\in perm([1,d])$, all the possible permutation of integers $\in [1,d]$ where $d$ is the layer size) while model updates in standard FL are from a \emph{continuous} space ($\in \mathbb{R}^d$).
In this approach, all the clients should learn a local rankings on their local data at the beginning of the learning, and send it to the server. Then the server clusters the rankings into $Q$ clusters to find the group ID of each client. This is just one time clustering, and throughout the \name learning, the server selects the local rankings for different group rank aggregation (majority voting) based on their group IDs (estimated with this approach). 




Algorithm~\ref{alg:IDEKmeans} in Appendix~\ref{Sec:unkownalgs} shows how the server can cluster the local rankings of $N$ clients into $Q$ groups. We adapt K-means clustering to cluster the rankings. In this algorithm, at first step (Algorithm~\ref{alg:IDEKmeans} line 3), we are choosing $Q$ random rankings as our initial $Q$ clusters, called centroids. Then we assign the cluster ID of the closest centroid for all the $N$ local rankings (Algorithm~\ref{alg:IDEKmeans} line 7-10). To determine the distance of two rankings, we use Spearman rank distance in which the distance between two rankings of $R_1$ and $R_2$ is $D(R_1, R_2) = \sum_{\ell\in[L]} \sum_{i \in [n_{\ell}]} |R_1[i]-R_2[i]|$ where $R_1[i]$ shows the rank of parameter $i$th in ranking $R_1$, $L$ is the number of layers in the network, and $n_{\ell}$ shows the number of parameters in layer $\ell$.
In next step (Algorithm~\ref{alg:IDEKmeans} line 11), we are updating the centroid of each cluster by applying majority vote on the ranking inside each cluster. We repeat this process for $T$ iterations to find final $Q$ groups of rankings. 
% , and we do the same thing by assigning the rankings by measuring the distance to each centroid.
% In following, we explain how to measure the distance between two rankings, and how to calculate the centroid of each cluster. 


% \paragraphb{Distance between two local ranking: }
% Spearmans distance: $D(R_1, R_2) = \sum_{\ell\in[L]} \sum_{i \in [n_{\ell}]} |R_1[i]-R_2[i]|$
% where $R_1[i]$ and $R_2[i]$ means the rank of the parameter ith in ranking $R_1$ and $R_2$. 
% % \begin{align}\label{eq:optimization}
% %     D(R_1, R_2) = \sum_{\ell\in[L]} \sum_{i \in [n_{\ell}]} |R_1[i]-R_2[i]|
% % \end{align}



% \paragraphb{Calculating the centroids of Ranking clusters}
% New centroid: we use the Rank aggregation method introduced in FRL to calculate the centroid.

% Please note that for finding the best group ID, there is no need to send all the rankings to the clients. As we mentioned before, each FSL model is a binary mask of '0's and '1's. So a client only receive the binary masks of the learned groups so far to decide which group it belongs to. 
% \vspace*{-6pt}
\subsection{Client-side:  Lowest Loss}
% \vspace*{-6pt}
In this approach, each client estimates its group ID by choosing the group that its binary mask produces the lowest loss. Thus, in each \name round, the server broadcasts all the binary masks related to existing groups ($M_{g, q \in [Q]}^t$), and each selected client calculates the loss for each binary mask on its training data. Algorithm~\ref{alg:IDE} line 2-4 in Appendix~\ref{Sec:unkownalgs} shows this approach. This approach was used by IFCA~\citep{ghosh2020efficient}, where in their algorithm in each training round, the server broadcasts all the model parameters to clients, and then they can find the lowest loss group. Note that our \name, compared to IFCA, needs $\times 32 (\times 64)$ less download bandwidth in each round because it is working on the binary masks.  




% \paragraphb{Problem Formulation} We try to partition clients in $q$ clusters, and train a separate model for each cluster, hence our optimization would be $\min_{h_1, ..., h_q} \sum_{u=1}^n \lambda_u \min_{j\in[q]} L_{D_u^{tr}} (h_j)$.

% % \begin{align}\label{eq:optimization}
% %     \min_{h_1, ..., h_q} \sum_{u=1}^n \lambda_u \min_{j\in[q]} L_{D_u^{tr}} (h_j)
% % \end{align}

% where $\lambda_u$ shows the importance of the $u^{th}$ user in empirical risk minimization. It could be $\lambda_u=\frac{m_u}{m}$ which gives importance to each client based on the size of data it has possessed. Or it can be $\lambda_u=\frac{1}{n}$ which gives a similar importance to all the participating clients. We used the latter in our setting. 
% \vspace*{-6pt}
\subsection{Client-side: Entropy of the output}
% \vspace*{-6pt}
Binary masks enable us to utilize other approaches for group inference. In these approaches~\cite{wortsman2020supermasks}, the client can infer the group ID using gradient-based optimization to find a linear superposition of learned binary masks which minimizes the output entropy. 
~\citet{wortsman2020supermasks} proposed these solutions to learn multiple tasks without catastrophic forgetting in continual learning. 
% Fair FL is similar to multi-task learning as the different groups are trying to model different data distributions, so we can use these approaches to 
In these solutions, each client infers the group ID by choosing the most confident binary mask that produces more stable results. There are two variants of this approach as follows: 

\paragraphb{OneShot inference:} Algorithm~\ref{alg:IDE} line 5-9 in Appendix~\ref{Sec:unkownalgs} shows this approach. At \name training round $t$, the server broadcasts $Q$ leaned binary masks $M_{g,q\in[Q]}^{t}$ to the selected clients. Next, each client assigns a confidence coefficient ($\alpha_q$) to each binary mask. 
Each $\alpha_q$ represents how much the client is confident that $q$th binary mask is its match. 
Then it calculates the output of the model as the weighted superposition of these masks (i.e., $p(\alpha) = f \left(x, \theta^w \bigodot (\sum_{q=1}^{Q} \alpha_q M_{g,q}^{t})\right)$).
The $\alpha$ is initialized in a way that all the masks have equal chance ($\alpha_0[q] = \frac{1}{Q}$ for $q \in [Q]$).
Now, Each client tries to find the perfect $\alpha_q$ that minimizes the entropy of the outputs $H(p(\alpha))$ by applying gradient descent with respect to $\alpha$ just for one round, i.e., $\alpha \gets \alpha - \beta \triangledown_{\alpha} H(p(\alpha))$. 
In this approach, the client chooses the group ID $q$ that changing its confidence level ($\alpha_q$) has the most impact on the entropy of the output of mixed models, i.e., $\arg\max_{q} \left( - \frac{\partial H(p(\alpha)))}{\partial \alpha_q}\right)$.

% \begin{equation}
%     p(\alpha) = f \left(x, W \bigodot (\sum_{i=1}^{k} \alpha_i M^{i})\right)
% \end{equation}


% Correct mask $M_{g,j}^{t}$ should result in more confident output, so for the right mask, the entropy of the output will decrease. 


% \begin{equation}
% \alpha \gets \alpha - \beta \triangledown_{\alpha} H(p(\alpha))
% \end{equation}

 

% \begin{equation}
% \arg\max_{i} \left( - \frac{\partial H(p(\alpha)))}{\partial \alpha_i}\right)
% \end{equation}




\paragraphb{Binary Search:} Algorithm~\ref{alg:IDE} line 10-23 in Appendix~\ref{Sec:unkownalgs} shows this approach. In this approach, the client utilizes binary search to find the best group ID by removing half of the candidates at each step until one $\alpha_q$ remains nonzero which indicates the best candidate. 
The client calculates the $p(\alpha)$ for $\alpha$, then it applies the gradient descent with respect to $\alpha$ on entropy of $p(\alpha)$. Next, the client eliminates half of the coefficients where they produce gradients less than the median of the gradients.  

% % \begin{wrapfigure}{r}{0.9\textwidth}
% % \centering
% % \vspace{-20pt}
% % \begin{figure}[H]
% \begin{table}
% \caption{Comparing time complexities of ID estimation approaches} \label{tab:comm}
% \centering
% % \setlength{\extrarowheight}{0.05cm}
% \footnotesize
% \begin{tabular} {c|c|c}
%   \hline
%   \multirow{1}{*}{Approach }  & Time Complexity & Additional Communication Complexity \\ \hline
%   Lowest Loss Method & O(k) forward passes & O($k \times M$) \\ \hline
%   Binary Search & O($\log k$) forward and backward passes & O($(k \times M$)\\ \hline
%   OneShot inference & O(1) forward and backward passes & O($k \times M$)\\ \hline
%   K-Means Clustering on Local Rankings & O(1) forward and backward passes & O(1) \\ \hline
% \end{tabular}
% \end{table}
% % \vspace{-20pt}
% % % \end{figure}
% % \end{wrapfigure}


 














==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/conclusion.tex <==
\vspace{-5pt}
\section{Conclusions}
% \vspace*{-6pt}
In this paper, we look at the fairness issue in FL with two different lenses. First we define equality and equity as fairness in user-level and group-level, respectively. 
We designed a novel collaborative learning algorithm, called \textbf{E}qual and \textbf{E}quitable \textbf{F}ederated \textbf{L}earning (\name) to achieve both equality and equity.
We validate the efficiency and fairness of \name in different real-world FL applications, and show that \name outperforms existing baselines in terms of the resulting efficiency, fairness of different groups, and fairness among all individual clients.


% We propose \emph{\textbf{F}ederated \textbf{S}upermask \textbf{L}earning} (FSL) where clients find a \emph{subnetwork} within a randomly initialized neural network, \emph{without} training the weights of the network. 
% Our extensive evaluation demonstrated FSL can provide better communication cost and more robustness to untargeted poisoning attacks compared to existing FL compressors and Byzantine-robust aggregation rules.


% https://umass-amherst.zoom.us/j/97936219914

\section*{Acknowledgements}
This work was supported by NSF grant 2131910. 

==> vxtknzbcybtgwndxcrkcndnccsnsxmjw/intro.tex <==
% \vspace*{-6pt}
\section{Introduction}
% \vspace*{-6pt}
%FL
% Federated Learning (FL) is an increasingly popular type of distributed learning which allows mutually untrusted clients to collaboratively train a common machine learning model without sharing their private/proprietary training data with each other.
Federated Learning (FL) is an emerging AI technology where \emph{clients} collaborate to train a shared model, called the \emph{global model}, without explicitly sharing their local training data. FL training involves a \emph{server} which collects model updates from selected FL clients in each round of training, and uses them to update the global model. 
%Fairness
In FL, the performance of the global model varies across the clients due to heterogeneity in the data that each client owns. 
This concern is called \emph{representation disparity}~\cite{hashimoto2018fairness} and results in unfair performance gaps for the participating clients. That is, although the accuracy may be high on average, some tail user whose data distribution differs from the majority of the clients is likely to  receive a much lower performance compared to the average. 

In this work, we look at FL fairness with two different lenses: \textbf{a)} \emph{Equality}: whose goal is providing similar performances for all  individual clients; \textbf{b)} \emph{Equity}: whose goal is providing similar performances across all  groups of clients (i.e., groups of majority and minority), where 
a group is defined as a set of clients with similar data distributions. 
The key question we try to answer is: \emph{Can we design an efficient federated learning algorithm that achieves both equality and equity concurrently?}


% Clients with same data distribution should find each other and help to train a global model. 


Due to the heterogeneity in clients’ data distributions, one single model cannot represent all the clients equally. 
There is a \emph{trade-off} between training one global model and multiple global models; if we  train one global model all the clients can utilize each other's knowledge, however it will be biased towards whom that have the majority of the population. On the other hand, if we train multiple  models (e.g., as in IFCA~\cite{ghosh2020efficient}, HypCluster~\cite{mansour2020three} and MOCHA~\cite{Smith17}), we improve fairness, but each global model will lose the knowledge from excluded clients.  
To get the best of both worlds, we present \textbf{E}qual and \textbf{E}quitable \textbf{F}ederated \textbf{L}earning (\name), a novel FL algorithm to achieve both equality and equity.
In \name, we train multiple global models, but in each round we combine all of the models into one global model to take advantage of the knowledge of all client groups. 

% \red{you dont need to refer to FRL directly. Just say that the idead of useing ranks has been suggested in prior work. don't make FRL a key prior work; it is not accepted anywhere}

The key insight used in \name is converting the problem of model weight optimization (in standard FL) to the problem of ranking model edges (a technique recently proposed in \cite{mozaffari2021frl}). 
Therefore, in each round of \name training, the clients and the server exchange rankings for the edges of a randomly initialized neural network (called \emph{supernetwork}), as opposed to exchanging parameter gradients.
More specifically, each \name client computes the importance of the edges within a randomly initialized neural network (called supernetowrk) on their local data, represented by a ranking vector. Next, \name server uses a majority voting mechanism to aggregate the collected local rankings into multiple global rankings based on the index of group they belong to. Finally, the \name server aggregates all the group rankings into one global ranking for next round of training. Applying the majority vote on the group rankings instead of all the local rankings helps  \name  enforce equity because each group has an equal vote to influence the global model. To provide equality in \name, if a client wants to use the model in a downstream task, they use their own group global ranking, instead of the global ranking, which is a better representation model for the client and its groupmates. 
% The global ranking is just for training, and group rankings will be used in downstream tasks.


Our ranking-based FL training  enables attractive fairness properties, as shown through our experiments, which is intuitively due to the following reason: 
% \red{the following reasons are too vague. please make more clear and more high level}
In rank-based federated learning, each client computes a local ranking (i.e., a permutation of integers $\in [1,d]$ where $d$ is the layer size), so each local ranking has a fixed norm (i.e., $\sqrt{1^2+2^2+...+d^2}$). 
This fixed norm of local updates makes the rank aggregation more fair as each local ranking has the same impact on the aggregated global ranking.
On the other hand, in standard FL, when the server aggregates the local model updates into the global model, each local update has a different impact on the global model (because of their different $l_2$ norms). For example in FedAvg, the server averages the parameter updates for the $d$ dimensions, therefore a large parameter update has more influence on the final average compared to a small parameter update. 

% \textbf{I)} each local ranking has same impact on the global ranking because  while each local update in standard FL has a different impact on the global model since they have different norms. \textbf{II)} Rank aggregation methods gives equal contribution to each ranking to produce the global ranking.  
% In stanadard FL, the $\ell_2$ norm of different model updates are different, so 
% In our experiments, we notice that the $l_2$ norm of the clients' updates is different which shows the impact of these updates would be different on the aggregated global model.


% What enables us to design FFRL is a novel learning paradigm called Federated Rank Learning (FRL)~\cite{mozaffari2021frl}. FRL reduces the space of client updates from model parameter updates (a continuous space of float numbers) in standard FL to the space of parameter rankings (a discrete space of integer values). 
% In each round of FRL, the clients and the server exchange rankings where a ranking is a  permutation of integers $\in [1,d]$ where $d$ is the size of a layer.

% We use rankings in FFRL instead of weight updates because rankings have potential fairness features:

%FRL
%  is a novel learning paradigm in which the clients compute a local ranking of parameters in a randomly initialized network, called supernetwork, compared to local parameter weight updates in standard FL. A ranking is a  permutation of integers $\in [1,d]$ where $d$ is the size of layer.
% Therefore, 






% Another feature of binary masks is that we can choose the right binary mask by applying novel technique~\cite{supsup} to find a mask with minimum entropy of the output using one shot inference. 









% \paragraphb{Equity can hurt the motivation of majority groups to participate in FL.} Equity is not the main goal of existing distributed learning systems because it can hurt the motivation of the majority of clients to  participate in the FL. If we have a learning algorithm that provides equity, it has this constraint to allow the same contribution from all groups (i.e., majorities and minorities). This comes with the price of reducing the performance of the majorities, which can demotivate them to participate to learn a model. 


% Therefore, we design \textbf{E}qualized \textbf{F}air \textbf{F}ederated \textbf{R}ank \textbf{L}earning (E-FFRL) to address both equality and equity in FL. In E-FFRL, each client gets its own group global ranking, instead of the global ranking, which is a better representation model for the client and its similar peers in that group.  
% \red{why do you give it a new name? why do you need to have both E-FFRL and FFRL? you just need to present one system and you can discuss how to tune its performance for different objectives. Also, above you said FFRL is designed to privde both equity and equality}

\paragraphb{\name when the group IDs are unknown.} In many applications, clients may be unaware of their protected attributes (i.e., the group they belong to). We propose one approach on server-side and three approaches on client-side for inferring  group IDs. To  infer the group IDs on the server-side, we propose to use a rank clustering approach to cluster  clients into groups.
Moreover, a client can also infer its group IDs by picking the right group based on their local training data. Using rankings allows us to exchange only the binary masks produced by each group ranking which lowers the communication cost compared to prior works.
Each client can pick the right binary mask based on three approaches. First, each client can pick the binary mask that produces the smallest loss. Binary masks also enable the clients to find their matching group by a new novel idea from~\cite{wortsman2020supermasks}, where clients can infer the group ID using gradient based optimization to find a linear superposition of learned masks which minimizes the output entropy. We propose two variants of this approach, one based on a binary search and the other using OneShot optimization.
% \red{i dont see "four" approaches here!}





\paragraphb{\em Empirical results:}
We experiment with three datasets in real-world heterogeneous FL settings and show that \name can help clients from both majority and minority groups, while q-FFL~\cite{li2019fair}, state-of-the-art fair FL, improves equality by helping the majorities and ignoring the minorities.
Since there are no existing distributed datasets containing different groups of clients with different data distributions, 
we create a new dataset, called FairMNISTRotate, to evaluate  equality and equity in FL applications. FairMNISTRotate represents 10 different handwriting styles, produced by rotating samples from the MNIST dataset. 
For FairMNISTRotate,
% \red{you have not even introduced this dataset. }
 q-FFL reduces the variance of accuracies for all  clients by 4\% while it increases the variance between groups by 81\% compared to FedAvg. On the other hand, our algorithm  reduces the variance of both clients and groups by 93\% and 95\% respectively compared to FedAvg. That is, \name improves both equity and equality, unlike prior fair FL algorithms. 

% Previous works, IFCA~\citep{ghosh2020efficient} or HypCluster~\citep{mansour2020three} separated train multiple models, also MOCHA~\cite{Smith17} and q-FFL~\cite{li2019fair} tries to \textbf{(3)} 

